Inferring Network Structure From Data

Networks are complex models for underlying data in many application domains. In most instances, raw data is not natively in the form of a network, but derived from sensors, logs, images, or other data. Yet, the impact of the various choices in translating this data to a network have been largely unexamined. In this work, we propose a network model selection methodology that focuses on evaluating a network's utility for varying tasks, together with an efficiency measure which selects the most parsimonious model. We demonstrate that this network definition matters in several ways for modeling the behavior of the underlying system.

==> intro_icdm.tex <==
\section{Introduction}

%Networks are models representing relationships between entities: individuals, genes, documents and media, language, products etc. We often assume the expressed or inferred edge relationships of the network are correlated with the underlying behavior of individuals or entities, reflected in their actions or preferences over time. 

%On some problems, the correspondence between observed behavior and network structure is well-established. For example, simple link-prediction heuristics in social networks tend to perform well because they correspond to the social processes for how networks grow \cite{Adamic2003}. However, content sharing in online social networks shows that `weak' ties among friends account for much of the influence on users \cite{Bakshy:2012:RSN:2187836.2187907}. For these different tasks, the same friendship network ``as-is'' is a relatively better \emph{model} for predicting new links than predicting content sharing. Learning an \textit{alternative} network representation for content sharing better predicts this behavior and is more informative of the relevant relationships for one task against another.

%Why should we learn a network representation at all? First, a \textit{good} network for a particular predictive task will perform better than methods over aggregate populations. Otherwise, edge relationships are not informative with respect to our purpose. Evaluating network models against population methods measures whether there is a network effect at all within the underlying data. In addition, network edges are \textit{interpretable} and suitable for descriptive analysis and further hypothesis generation. Finally, a good network model \textit{generalizes} several behaviors of entities observed on the network, and we can evaluate this robustness under a shared representation. For these reasons, we should learn a network representation if we can evaluate `which' network is useful and whether there is the presence of any network on the underlying data. 

%Much of the previous work focuses on method development for better predictive accuracy on a \textit{given network}. However, predictive method development on networks treats the underlying network representation as independent of the novel task method, rather than coupled to the \textit{network representation} of underlying data. Whether network structure is given or inferred, choosing the best representation affects subsequent tasks and questions on the network. How do we measure the effect of these network modeling choices on common and general classes of predictive tasks (e.g. link prediction, label prediction, influence maximization)? 

%Our work fills this methodological gap, coupling general network inference models from data with common predictive task methods in a network model selection framework. This framework evaluates both the definition of an edge, and the `neighborhood' function on the network most suitable for evaluating various tasks. 

\section{Related Work}

Our work is primarily related to research in relational machine learning, and network structure inference.

Relational learning in networks uses correlations between network structure, attribute distributions, and label distributions to build network-constrained predictive methods for several types of tasks. Our work uses two fundamental relational learning tasks, link prediction and collective classification to evaluate network models inferred from data.

The link prediction task \cite{Hasan2011} predicts edges from `local' information in the network. This is done by simple ranking, on information such as comparisons over common neighbors \cite{Adamic2003}, higher-order measures such as path similarity \cite{Liben-Nowell2007}, or learning edge/non-edge classification as a supervised task on extracted edge features \cite{al2006link, Gong:2014:JLP:2611448.2594455}.

The collective classification task \cite{london2014collective, sen:aimag08} learns relationships between local neighborhood structure of labels and/or attributes \cite{McDowell:2013:LAR:2505515.2505628} to predict unknown labels in the network. This problem has been extended to joint prediction of edges \cite{4476695}, and higher-order joint prediction \cite{namata:tkdd15}. Our work does not extend these methods. Where suitable, more sophisticated predictive task methods and higher-order joint methods may be used for evaluating network models and model selection.

Network structure inference \cite{2016arXiv161000782B, Kolaczyk2014} is a broad area of research aimed at transforming data on individuals or entities into a network representation which can leverage methods such as relational machine learning. Previous work spans numerous domains including bioinformatics \cite{ZhangHorvath2005}, neuroscience \cite{Sporns2014}, and recommender systems \cite{McAuley:2015:INS:2783258.2783381}. Much of this work has domain-driven network model evaluation and lacks a general methodology for transforming data to useful network representations.

Models for network inference are generally either parametric, or similarity-based. Parametric models make assumptions of the underlying data distribution and learn an edge structure which best explains the underlying data. For example, previous work has modeled the `arrival time' of information in a content network with unknown edges, where rates of transmission are the learned model \cite{Gomez-Rodriguez:2012:IND:2086737.2086741, Myers2010}. 

Several generative models can sample networks with correlations between attributes, labels, and network structure, and can estimate model parameters from data. These include the Attributed Graph Model (AGM) \cite{Pfeiffer:2014:AGM:2566486.2567993}, Multiplicative Attribute Graph model (MAG) \cite{Kim2012}, and Exponential Random Graph Model (ERGM) \cite{Robins2007}. However, these models are typically not estimated against a task of interest, so while it may fit our modeling assumption, it may not model the subsequent task; our proposed methodology straightforwardly accepts any of these models estimated from data.

Similarity-based methods tend to be ad-hoc, incorporating domain knowledge to set network model parameters. Recent work on task-focused network inference evaluates inferred network models according to their ability to perform a set of tasks \cite{DeChoudhury:2010:IRS:1772690.1772722}. These methods often have a high sensitivity to threshold/parameter choice, and added complexity of interactions between network representations and task models. Our work identifies these sensitivities, and yields robust model selection over several stability criteria.


\section{Contributions}
We present a general, modular methodology for model selection in task-focused network inference. Our work:
\begin{compactitem}
    \item identifies constituent components of  the common network inference workflow, including network models, tasks, task neighborhood functions, and measures for evaluating networks inferred from data,  
    \item uses fundamental, interpretable network models relevant in many application domains, and fundamental tasks and task \textit{localities} measuring different aspects of network-attribute correlations,
    \item presents significance, stability, and null-model testing for task-focused network model selection on three online user activity datasets.
\end{compactitem}

Our work focuses on process and methodology; the development of novel network models and task methods are complimentary but distinct from this work. Our work demonstrates that network representation learning is a crucial step for evaluating predictive methods on networks. 


==> methods_icdm.tex <==
\section{Methods}


\subsection{Task-Focused Network Inference and Evaluation}

\begin{figure*}[ht]
\centering
  \includegraphics[width=\bannerwidth\textwidth]{figs/icdm/schematic}
  \caption{A schematic of the model selection methodology. (a) Individual node attributes and labels are provided as input, an edge-set may be provided (dashed edges). (b) A collection of networks are inferred from functions on attributes and labels, outputting an edge-set. (c) For each network model, we build a classification method on attributes and labels for each node of interest (black) constraining node-attribute and node-label available to the method (cyan) according to constraints from the network structure. These `global', `meso', and `local' methods produce prediction output for some task (e.g. link prediction, collective classification). (d) we select a network representation subject to performance for the given task.} 
  \label{fig:overview}
\end{figure*}

Model selection for task-focused network inference learns a network model and associated parameters which perform a task or set of tasks with high precision. We learn joint relationships between node attribute vectors and some target label (e.g. node behavior) of interest.

Figure \ref{fig:overview} presents a high-level schematic of our methodology and the constituent components of task-oriented network inference problems. First, (a) our data is a collection of attributes and labels associated with discrete entities. Edges are optionally provided to our methodology, indicated by dashed lines. Edges may be entirely missing or one or several edge-sets. In all these cases we evaluate each edge-set as one of many possible network `models.' Attributes are any data associated with nodes (and/or edges) in the network. These are often very high dimensional, for example user activity logs and post content in social networks, gene expression profiles in gene regulatory networks, or full document text and other metadata in document, video or audio content networks.

Labels are a notational convenience denoting a specific attribute of predictive interest. Labels are typically low-cardinality fields (e.g. boolean) appropriate for supervised classification methods. Our methodology accepts (and prefers) \textit{multi}-labeled networks. This simply indicates multiple fields of predictive interest. For example, we induce labels as an indicator for whether a user is a listener or a viewer of `this' music or movie genre, given by historical activity data over many such genres. Multiple sets of these labels more robustly evaluate whether attribute relationships in the fixed underlying network model generalize to these many `behaviors.' 

Second, in Figure \ref{fig:overview} (b) we apply several fundamental network inference models. These are modular and can be specified according to the domain. These models are either parametric statistical methods, or functions on similarity spaces, both of which take attributes and/or labels as input and produce an inferred edge-set. Note in \ref{fig:overview} (b) that the stacked edge-sets vary. 

Third, in Figure  \ref{fig:overview} (c) for every node of interest (black) for some predictive task, we select sets of nodes (cyan, grey nodes excluded) and their associated attributes and labels according to various \textit{task locality functions} (i.e. varying `neighborhood' or network query functions). These functions include globally selecting the population of all nodes, sampling nodes from within `this' node's community by the output of some structural community method, an ensemble of a small number of nodes according to attribute or network ranking (e.g. degree, centrality), or local sampling by simple network adjacency or some other ordered traversal. 

Once selected, the associated attributes and labels of the cyan nodes yield a supervised classification problem predicting label values from attribute vectors, using a predictive task model of interest. Several fundamental prediction problems fit within this supervised setting. For example, link prediction can use positive (edge) and negative (non-edge) label instances rather than learning classifiers on the input labelsets. 

We evaluate network models (b) over the collection of its task methods and varying localities (c) to produce Figure \ref{fig:overview} (d), some predictive output (e.g. label prediction, shown here). The model and locality producing the best performance is selected. Finally, we further evaluate the stability and significance of our selected model over the collection of possible models. 

Below, we infer networks to identify listeners/reviewers of music genres, film genres, and beer types in three user activity datasets: Last.fm, MovieLens and BeerAdvocate, respectively.

%\subsubsection{Attributed Networks and Labeled Networks}

%Our methodology focuses on attributed networks. 




% This particular network inference problem corresponds to learning the unknown label function, represented on the learned network structure.


%Our framework accepts a set of network models which may include any observed \textit{explicit} networks, which are treated as a possible model. Our framework also accepts multiple label-sets and task methods. The methodology performs model selection which is robust across these varying labelsets or tasks. 

\begin{algorithm2e}
  \SetAlgorithmName{Problem}
  \\
  \\
  \KwGiven{Node Attribute-set $A$, Node Label-sets $L^*$,\\ 
  Network model-set $\mathcal{M}_j \in M$ where $\mathcal{M}_j(A,L) \rightarrow E_j'$,\\  
  Task-set $ \mathcal{C}_k \in C$ where $ \mathcal{C}_k(E_j',A,L^*) \rightarrow P_{kj}'$}
  \KwFind{Network edge-set $E_j'$}
  \KwWhere{$\argmin_j \mathcal{L}(P, P_{kj}')$ on validation $P$}
  \caption{Task-Focused Network Inference Model Selection}
  \label{p:networkinference}
\end{algorithm2e}

Problem \ref{p:networkinference} gives a concise specification of our model selection framework, including inputs and outputs. Given individual node-attribute vectors $\vec{a}_i \in A$, where `$i$' corresponds to node $v_i$ in node-set $V$, and a collection of node-labelsets $L \in L^*$, where $l_i \in L$ the label of node $v_i$ in a single labelset $L$, our general task-focused network inference framework evaluates a set of possible network models $M =\{\mathcal{M}_1...\mathcal{M}_n\}$  where each $\mathcal{M}_j: \mathcal{M}_j(A,L) \rightarrow E_j'$ produces a network edge-set $E_j'$.\footnote{Notation: capital letters denote sets, lowercase letters denote instances and indices. Primes indicate \emph{predicted} and inferred entities. Greek letters denote method parameters. Script characters (e.g. $\mathcal{C}()$) denotes functions, sometimes with specified parameters.} 

These instantiated edge-sets are evaluated on a set of inference task methods $C = \{\mathcal{C}_1...\mathcal{C}_m\}$ where each $\mathcal{C}_k$ produces $P_k'$, a collection of predicted edges, attributes, or labels  depending on context: $\mathcal{C}_k(E_j',A,L^*) \rightarrow P_{kj}'$. We evaluate a $P'$ under loss $\mathcal{L}(P, P')$, where $P$ is the validation or evaluation data. We select $\mathcal{M}_{\mathrm{select}} = \argmin_j \mathcal{L}(P, P_{kj}')$ based on performance over $C$ and/or $L^*$. Finally, we evaluate generalized performance of this model choice.

Our methodology can be instantiated under many different network model-sets $M$, task methods $C$, and loss functions $\mathcal{L}()$. We present several fundamental, \textit{interpretable} modeling choices common to many domains. All of these identified choices are modular and can be defined according to the needs of the application. For clarity, we refer to the network representation as a \textit{model}, and the subsequent task as a method, because we focus on \textit{model selection} for the former.

\subsection{Network models}

Network models are primarily parametric under some model assumption, or non-parametric under a similarity space. We focus on the latter to avoid assumptions about joint attribute-label distributions. 

We present two fundamental similarity-based network models applicable in most domains: the k-nearest neighbor (KNN) and thresholded (TH) networks. Given a similarity measure $\mathcal{S}(\vec{a}_i, \vec{a}_j) \rightarrow s_{ij}$ and a target edge count $\lambda$, this measure is used to produces a pairwise attribute similarity space. We then select node-pairs according to:

%\footnote{Sub-quadratic approximation of these similarity spaces vary by measure, and is outside the scope of our methodology.}

\begin{compactitem}
	\item $k$-nearest neighbor $\mathcal{M}_{\mathrm{KNN}}(A, \mathcal{S}, \lambda)$: for a fixed $v_i$, select the top $\lfloor\frac{\lambda}{|V|}\rfloor$ most similar $\mathcal{S}(\vec{a}_i, \{A \setminus \vec{a}_i\})$. In directed networks, this produces a network which is $k$-regular in out-degree, with $k=\lfloor\frac{\lambda}{|V|}\rfloor$.
	\item Threshold $\mathcal{M}_{\mathrm{TH}}(A, \mathcal{S}, \lambda)$: for \emph{any} pair $(i,j)$, select the top $\lambda$ most similar $\mathcal{S}(\vec{a}_i, \vec{a}_j)$
\end{compactitem}

For a fixed number of edges, the varying performance of these network models measures the extent that absolute similarity, or an equal allocation of modeling per node produces better predictive performance.

\subsubsection{Node attribute similarity measures}

When constructing a network model on node attribute and label data, we compare pairwise attribute vectors by some similarity and criteria to determine an edge. These measures may vary greatly according to the nature of underlying data. Issues of projections, kernels, and efficient calculation of the similarity space are complimentary to our work, but not our focus.

Our example applications focus on distributions of item counts: artist plays, movie ratings, beer ratings, where each attribute dimension is a unique item, and the value is its associated rating, play-count etc. Therefore we measure the simple `intersection' of these vectors. 

Given a pair of attribute vectors $(\vec{a}_i, \vec{a}_j)$ with non-negative elements, intersection $\mathcal{S}_{INT}()$ and normalized intersection $\mathcal{S}_{INT-N}()$ are given by:
\begin{equation}
    \begin{aligned}
	\mathcal{S}_{INT}(\vec{a}_i, \vec{a}_j) = \sum\nolimits_d \mathrm{min}(a_{id}, a_{jd}) \\
	\mathcal{S}_{INT-N}(\vec{a}_i, \vec{a}_j) = \frac{\sum\nolimits_d \mathrm{min}(a_{id}, a_{jd})}{\sum\nolimits_d \mathrm{max}(a_{id}, a_{jd})} 	
	\end{aligned}	
\end{equation}

These different similarity functions measure the extent that \textit{absolute} or \textit{relative} common elements produce a better network model for the task method. Absolute similarity favors more active nodes which are highly ranked with other active nodes before low activity node-pairs. For example, in our \lfm application below, this corresponds to testing whether the total count of artist plays between two users is more predictive than the \textit{fraction} of common artist plays.

\subsubsection{Explicit network models}

Our methodology accepts observed, explicit edge-sets (e.g. a given social network) not constructed as a function of node attributes and labels. This allows us to test given networks as fixed models on attributes and labels, for our tasks of interest. 

\subsubsection{Network density}

We evaluate network models at varying density, which has previously been the primary focus of networks inferred on similarity spaces \cite{Myers2010, DeChoudhury:2010:IRS:1772690.1772722}. When evaluating network models against a given explicit network, we fix density as a factor of the explicit network density (e.g. $0.75\times \mathrm{d}(E)$). Otherwise, we explore sparse network settings. We don't impose any density penalty, allowing the framework to equally select according to predictive performance.

% \subsection{Tasks for Evaluating Network Models}

% We evaluate network models on two fundamental network tasks: collective classification and link prediction. 

% \subsubsection{Collective classification (CC)} The collective classification problem learns relationships between network edge structure and attributes and/or labels to predict label values \cite{sen:aimag08, 4476695}. This task is often used to infer unknown labels on the network from `local' discriminative relationships in attributes, e.g. labeling political affiliations, brand or media preferences.

% Given an edge-set $E'$, a neighborhood function $\mathcal{N}(E',i)$, and node-attribute set $A$, the collective classification method $\mathcal{C}_{\mathrm{CC}}(A_{\mathcal{N}(E', i)}, L_{\mathcal{N}(E',i)}, \vec{a}_i) \rightarrow l_i'$ trains on attributes and/or labels in the neighborhood of $v_i$ to predict a label from attribute \emph{test} vector $\vec{a}_i$. 

% We use this task to learn network-attribute-label correlations to identify \textit{positive} instances of rare-class labels. As an oracle, we provide the method only these positive instances because we want to learn the true rather than null association of the label behavior. Learning positive instances over many such labelsets allows us to robustly evaluate learning on the network model under such sparse labels.

% \subsubsection{Link prediction (LP)}

% The link prediction problem \cite{Liben-Nowell2007} learns a method for the appearance of edges from one edge-set to another. Link prediction methods can incorporate attribute and/or label data, or using simple structural ranking \cite{Adamic2003}.

% Given a training edge-set $E'$ induced from an above network model, a neighborhood function $\mathcal{N}(E', i)$, and a node-attribute set $A$, we learn edge/non-edge relationships in the neighborhood as a binary classification problem on  edge/non-edge attribute vectors, $\vec{a}_{jk}$ where  $(j,k) \in \mathcal{N}(E', i)$. On input test attributes $\vec{a}_{jk}$, the model produces an edge/non-edge label: $\mathcal{C}_{\mathrm{LP}}(A_{\mathcal{N}(E', i)}, \vec{a}_{jk}) \rightarrow l_{jk}'$. For our applications, the simple node attribute intersection is suitable to construct edge/non-edge attributes: $\vec{a}_{jk} = \underset{d=1...|\vec{a}_j|}{\mathrm{min}}(a_{jd}, a_{kd})$. 

\subsection{Task Locality}
\label{subsec:task_locality}
Both of the above tasks are classifiers that take attributes and labels as input, provided by the neighborhood function $\mathcal{N}(E', i)$. However, this neighborhood need not be defined as network adjacency. We redefine the neighborhood function to provide each task method with node/edge attributes selected at varying locality from the test node. These varying localities give interpretable feedback to which level of abstraction the network model best performs the task of interest. We propose four general localities:

\subsubsection{Local}

For CC, local methods use simple network \textit{adjacency} of a node $v_i$. For LP, local methods use the \textit{egonet} of a node $v_i$. This is defined as an edge-set from nodes adjacent to $v_i$, plus the edges of these adjacent nodes. Non-edges are given by the compliment of the egonet edge-set. We also evaluate a breadth-first-search neighborhood (BFS) on each model, collecting $k$ (=200) nodes encountered in the search order.

\subsubsection{Community}

We calculate structural community labels for each network using the Louvain method \cite{ICT4DBibliography2429}. We sample nodes and edges/non-edges from the induced subgraph of the nodes in the `test' node's community. 

\subsubsection{Ensemble}

We select $k$ (=30) nodes according to some fixed ordering. These nodes become a collection of locally-trained task methods. For each test node, we select the KNN (=3) ensemble nodes according to the similarity measure of the current network model, and take a majority of their prediction.

We use decreasing node-order on (1) Degree, (2) Sum of attributes (i.e. most `active' nodes), (3) Unique attribute count (i.e. most diverse nodes), and (4) Random order (one fixed sample per ensemble).

Ensembles provide `exemplar' nodes expected to have more robust local task methods than those trained on the test node's neighborhood, on account of their ordering criteria. These nodes are expected to be suitably similar to the test node, on account of the KNN selection from the collection. 
 
\subsubsection{Global}

We sample a fixed set of nodes or edges/non-edges without locality constraint. This measures whether the network model is informative at all, compared to a single global classification method. This measures the extent that a task is better represented by aggregate population methods than encoding local relationships. Although models with narrower locality are trained on less training data, they can learn local heterogeneity of local attribute relationships which may confuse an aggregated model. 

\subsection{Classification Methods}

For all different localities, both of our tasks each reduce to a supervised classification problem. For the underlying classification method, we use standard linear support vector machines (SVM), and random forests (RF). These are chosen due to speed and suitability in sparse data. Absolute predictive accuracy is not the primary goal of our work; these methods need only to produces consistent network model ranking over many model configurations. 

\subsection{Network Model Configurations}
We define a network model configuration as a combination of all specified modeling choices: network model, similarity measure, density, task locality, and task method. Each network model configuration can be evaluated independently, meaning we can easily scale to hundreds of configurations on small and medium-sized networks. 

